Understanding Acoustic Patterns of Human Teachers Demonstrating Manipulation Tasks to Robots

Humans use audio signals in the form of spoken language or verbal reactions effectively when teaching new skills or tasks to other humans. While demonstrations allow humans to teach robots in a natural way, learning from trajectories alone does not leverage other available modalities including audio from human teachers. To effectively utilize audio cues accompanying human demonstrations, first it is important to understand what kind of information is present and conveyed by such cues. This work characterizes audio from human teachers demonstrating multi-step manipulation tasks to a situated Sawyer robot using three feature types: (1) duration of speech used, (2) expressiveness in speech or prosody, and (3) semantic content of speech. We analyze these features along four dimensions and find that teachers convey similar semantic concepts via spoken words for different conditions of (1) demonstration types, (2) audio usage instructions, (3) subtasks, and (4) errors during demonstrations. However, differentiating properties of speech in terms of duration and expressiveness are present along the four dimensions, highlighting that human audio carries rich information, potentially beneficial for technological advancement of robot learning from demonstration methods.

==> IROS 2022 arXiv 2/1-intro.tex <==
\section{Introduction}
\begin{comment}
\ess{consider deleting this paragraph entirely}
As personal robots become more prevalent in dynamic and  unstructured  human  environments,  they  will  come  to  interact with and  rely  more on end-users. A common approach for end-users to specify new tasks to autonomous agents is in the form of demonstrations.  This learning paradigm is called Learning from Demonstration (LfD) %or Imitation Learning (IL) 
\cite{argall2009survey, osa2018algorithmic}, where an agent learns by observing demonstrations of how to perform a task. This is more intuitive and natural for end-users compared to hand-designing reward functions 
for reinforcement learning.
However, complex and dynamic environments require large amounts of demonstrations, increasing the time and effort for human teachers.
For robots to be successfully deployed in complex environments, it is important that they can leverage as much information as possible from a user's demonstrations.
\end{comment}


Human speech or audio is a natural, low-effort and rich channel of communication \cite{oviatt2004we}. Typically, robot learning from demonstration (LfD) algorithms ignore information carried by a human teacher's audio cues%during a demonstration
, and only work with the state of the environment and 
the human teacher's actions \cite{argall2009survey, osa2018algorithmic}. Some prior works have leveraged gaze patterns of human demonstrators \cite{saran2018human,saran2020understanding,zhang2020human,saran2020efficiently}. However, to the best of our knowledge, human audio has been primarily unexplored in the context of learning from demonstration. 
A primary reason why incorporating this additional information has been challenging is the lack of understanding about how complex human audio signals are used and what they convey during demonstrations. 
%\as{A major challenge is also the feasibility and reliability of sensors and that verbal human descriptions of tasks are often erroneous and underspecified \cite{srimal2017deictic,gustavsson2017human,gross2017reliability}. Recent advancements in sensor technology, audio processing algorithms should address the first two. Even if underspecificied, there could be useful information which could be leveraged.}
Recent advancements in sensor technologies and speech processing algorithms~\cite{yu2016automatic} make it possible to extract informative features from human audio.
\textit{Raw} human audio carries more information than is present in a transcribed narration of textual words produced by an automatic speech recognition (ASR) system \cite{yu2016automatic}. Audio can contain information via spoken language, as well as out-of-vocabulary words not part of a natural-language learning corpus, disfluencies (restarts, repetitions, and self-corrections), filled pauses (`um', `uh'), hyperarticulations such as careful enunciation, slow speaking rate, increased pitch and loudness \cite{clark2002using}.
This work is a first step in analyzing 
how humans use unrestricted audio cues during demonstrations for multi-step manipulation tasks
---characterizing duration, prosodic features, and spoken words.

\begin{figure}
\centering
\subfigure[Kinesthetic Demonstration]{
\includegraphics[width=0.225\textwidth]{images/kt_speech_small.png}
}
\subfigure[Video Demonstration]{
\includegraphics[width=0.225\textwidth]{images/video_speech_small.png}
}
\caption{
(a) Kinesthetic demonstrations and (b) Video demonstrations along with unrestricted audio signals of human teachers are recorded for two manipulation tasks. %\as{Update with speech symbol.}
}
\vspace{-5mm}
\label{fig:sawyer}
\end{figure}

We work in a limited-data regime with an in-house dataset of demonstrations and accompanying human audio, collected via a human subjects study in a laboratory setting. With the help of human annotators, we characterize human speech via: (1) duration of speech in a demonstration, (2) annotated and computational prosodic features, (3) semantic content of words spoken during speech.
We analyze these features across different dimensions: (a) type of demonstration used (kinesthetic teaching using the robot's arm versus the human performing the task themselves), (b) the instruction given to a teacher about usage of speech during demonstrations (explicit narration instructions versus implicit indication to use speech), (c) presence or absence of relevant subtasks being executed, (d) presence or absence of errors during demonstrations. We find that users convey similar semantic concepts through spoken words across all four dimensions. However, we observe that teachers are more expressive but talk less densely during kinesthetic teaching compared to demonstrating the task themselves. Moreover, teachers are similarly expressive across audio usage instructions for a majority of acoustic features, but overall talk more when explicitly asked to do so.  
We also find that with a majority of acoustic features, teachers use speech more densely and more expressively during relevant subtask executions and in the absence of errors. However, some interesting speech features exist even in the absence of subtasks and in the presence of errors.

Finally, with a proof-of-concept experiment, we show that human acoustic features are useful to detect presence of relevant subtasks and errors during demonstrations. Taken together, our findings highlight that human speech carries rich information about demonstrations, which can be beneficial for technological advancement of robot learning algorithms in the future.

\begin{comment}
Most human speech during such demonstrations is not very expressive but rather descriptive. It is the presence and duration of speech that is most indicative of subtasks and errors during demonstrations.
\end{comment}

==> IROS 2022 arXiv 2/2-related.tex <==
\begin{figure}
\centering
\subfigure[Box Opening]{
\includegraphics[width=0.08\textwidth]{images/sawyer/box_start.jpg}
\includegraphics[width=0.08\textwidth]{images/sawyer/box_end.jpg}
}
\subfigure[Fruit Cutting]{
\includegraphics[width=0.13\textwidth]{images/sawyer/cutting-start.jpg}
\includegraphics[width=0.13\textwidth]{images/sawyer/cutting-end.jpg}
}
\caption{Start and end conditions of two manipulation tasks for which demonstrations are provided to a Sawyer robot.}
\label{fig:sawyer-tasks}
\vspace{-5mm}
\end{figure}

\section{Related Work}
%In relation to our work, we discuss prior works which  leverage human speech signals to enhance human-robot interaction as well as prior works which augment robot learning algorithms with audio signals including speech and environmental sounds. \sn{If you need space, you can delete this para.}

\begin{comment}
\subsection{Speech Usage during Human-Human Teaching}
Private speech studies among children have shown that talking aloud can have a positive effect on task learning \cite{teasley1995role, berk1999children, ericsson1984protocol}. Teasley et al. \cite{teasley1995role} describe that 
to manage coherence and activity simultaneously, partners must make utterances that signal intentions, current interpretations and expectations. Within the context of a shared problem-solving task, these utterances take the form of plans, strategies, and explanations.  
Duff et al. \cite{duff1985another} study the effect of non-native speaker dyads towards problem-solving tasks. They notice turn-taking patterns among people, which mostly consist of simple phrases -- questions, repetitions, reformulations, and explanations of various kinds. Pan et al. \cite{pan1996communicative} show that as children
become more communicative, 
parents produce fewer communicative acts as children begin to take up more of the conversational load during joint problem solving for various learning tasks. \as{Check again.} While these prior works have established theories about how humans talk during collaboration and learning with each other, we study the usage of one-directional speech as humans teach tasks to robots. \ess{I think you actually want to say something more like "this demonstrates that humans are used to talking during teaching; in this work we investigate what automatically-extractable information is available in that speech"}
\end{comment}

%\as{I would suggest to also include works on the analysis of audio cues in demonstrations from parents to children (e.g., Schillingmann et al., 2009 on acoustic packaging) which also analyze unrestricted audio signals in human tutoring. \cite{schillingmann2009computational}}




\subsection{Human Audio-assisted Human-Robot Interaction}

Scassellati et al. \cite{scassellati2009affective} showed that understanding emotion in the context of a conversation is an essential skill for keeping humans engaged when interacting with robots. They developed a service that helps a robot to recognize acoustic patterns in a human's tone of voice by classifying approving, neutral and prohibitive affects. Kim et al. \cite{kim2009people}
identified three phases during which humans use affective prosody during interactive reinforcement learning. These three phases are: direction (before the learner acts), guidance (as the learner indicates intent) and feedback (after the learner completes a task-action).  
Short et al. \cite{short2018detecting} used ratio of variances in raw speech features to detect contingent human responses to robot probes for open-world human-robot interaction. However, in comparison to the problem settings of 
these prior works,
%\cite{scassellati2009affective,kim2009people,short2018detecting}
 we focus on the learning from demonstration paradigm %. 
%Staudte et al. \cite{staudte2009visual} showed that speech and prosody features improve engagement for human-robot interaction. However, the emphasis was on speech generated by the robot. 
%In our work, we instead %directly study 
and characterize raw audio signals of human teachers to better understand the information present in this modality.
Work on infant-directed demonstrations~\cite{nagai2008toward} as well as robotics work inspired from infant-directed speech~\cite{nakamura2015constructing} highlights that the way that people talk to a robot could possibly help it learn more easily if they treat it like it is an infant, than if they spoke to it like it is an adult. However, this may not always be possible with a variety of commercialized robots not exhibiting infant-like appearances or personalities. In our work, we study how human demonstrators use unrestricted speech to teach robots which are not infant-like in appearance or behavior, to better inform how human audio cues could be leveraged for learning by a variety of robots. %a more scalable way.


\subsection{Human Audio-assisted Robot Learning}
Prior research in learning from demonstration 
has utilized human speech signals accompanying demonstrations, however with a restricted vocabulary of words used by the human teacher. Nicolescu et al. \cite{nicolescu2003natural} demonstrated the role of verbal cues both during demonstrations and as feedback from the human teacher during the agent's learning process, to facilitate learning of navigation behaviors on a mobile robot. However, they restricted human teachers to use a limited vocabulary of words to indicate relevant parts of the workspace or actions that a robot must execute. Similarly, 
Pardowitz et al. \cite{pardowitz2007incremental} used a fixed set of seven vocal comments which are mapped one-to-one with features relevant to the task 
to augment subtask similarity detection and learning of the task model from demonstrations 
for a simple table setting task. Prior work in reinforcement learning has also utilized a fixed vocabulary of words to record voice-based feedback for reward shaping~\cite{tenorio2010dynamic} and reinforcement learning ~\cite{kim2007learning}. Some works have also utilized sentiment analysis using natural language processing to aid reinforcement learning with the semantics of spoken words \cite{krening2016learning, krening2018newtonian}.
However, in our work, we use raw and unrestricted speech signals accompanying demonstrations to understand how human teachers convey information via audio.

==> IROS 2022 arXiv 2/3-approach.tex <==
\section{Methodology}


\begin{figure}
\centering
\subfigure[Natural Instruction Type]{
\includegraphics[width=0.225\textwidth]{images/annotations/user11_cutting_kt.png}
}
\subfigure[Narration Instruction Type]{
\includegraphics[width=0.225\textwidth]{images/annotations/user7_cutting_kt.png}
}

\caption{Subtasks, human  %audio 
utterances, and errors during demonstrations are shown on the top, middle, and bottom rows respectively during kinesthetic demonstrations for the fruit cutting task (each subtask category represented with a different color, all error categories represented by the same color). 
}
\vspace{-5mm}
\label{fig:seg_errors}
\end{figure}

To develop an understanding of complex audio signals from human teachers demonstrating manipulation tasks to an embodied robot, we aim to understand how three different acoustic properties (duration, prosody, semantic content) are used by human teachers across demonstration modalities, audio-usage instructions, relevant subtask segments, and errors during demonstrations.
To analyze this information, we conducted a user study (Sec. \ref{sec:user-study}) where human teachers demonstrate two multi-step manipulation tasks (Sec. \ref{sec:tasks}) to a Sawyer robot. 
We recorded audio data
along with visual state observations for two demonstration modalities --- kinesthetic teaching (KT) and video demonstrations (Sec. \ref{sec:system}).
Half of the participants were asked to explicitly narrate what they were doing as they demonstrated the task and the other half were only implictly told that the robot can watch and listen to them (instruction type).
To characterize audio utterances of human teachers accurately, we collected annotations for when teachers talk and what they conveyed through it. To understand how utterances relate to %multi-step 
task segments and errors during demonstrations, we also collected annotations for (1) subtask segment labels,  
(2) types of demonstration errors, and 
(3) characterizations of human speech accompanying subtasks and errors. 
Details about our annotation procedure are explained in Sec \ref{sec:annotation}.  
Finally, in light of recent LfD methods which (1) highlight that learning a separate policy for each subtask in a multi-step task is more efficient~\cite{kroemer2019review} and (2) utilize suboptimal demonstrations~\cite{osa2018algorithmic}, we analyze if human audio contains beneficial information for two related learning problems --- detecting the presence of subtasks and detecting the presence of demonstration errors. Through proof-of-concept experiments, we demonstrate that random forest classifiers can detect subtasks \& errors during demonstrations (Sec. \ref{sec:learning-method}) with a varied set of human acoustic features (Sec. \ref{sec:features}).%\footnote{Code: https://github.com/asaran/human-speech-demo-analysis}.




\subsection{Task Descriptions}
\label{sec:tasks}
The two household tasks relevant to personal robots that were used in our study are: (a) box opening and (b) fruit cutting (Fig.~\ref{fig:sawyer-tasks}). % The task layouts were kept roughly the same across all participants, but no markers were used to fix the locations of the objects. %are shown in Fig.\ref{fig:sawyer-tasks} (a), (b).
Each task consists of multiple subtasks performed in sequence to accomplish the overall goal. There could be pauses and errors during and between the execution of the subtasks. Details of the two tasks are as follows:
\subsubsection{Box Opening} A transparent box contains a green wooden object inside it. A circular button located in the center of the lid (covered with black paper) is pressed. This unlocks the lid from the box. The lifted circular part of the lid is then grasped to open the box. Then, the green wooden object is picked from inside the box and placed on the table. The lid is placed on top of the box. The circular button of the lid is pressed again to lock the box. Finally, the green object is picked from the table and placed on top of the black circular button of the lid. The goal is to perform the task without moving the box from its location on the table surface (Fig.~\ref{fig:sawyer-tasks}(a)). This is a multi-step pick-and-place task with a challenging maneuver of lifting an object from inside the box. This task is representative of several goal-oriented household tasks.

\subsubsection{Fruit Cutting}
A flat surface contains different colored wooden fruit pieces on it, along with an uncut wooden banana whose three pieces are stuck together with Velcro. A wooden knife is placed in a knife holder. The gripper of the knife is covered with foam so it can be easily grasped by the robot.
A slit with a black marking indicates where the robot's gripper can firmly grasp the knife. The knife is taken out of the knife holder, and then used to cut the banana into three pieces by making two cuts through the two Velcro attachments. Finally, the knife is placed back into the knife holder. The goal is to cut the banana without moving any other fruit on the wooden surface such that the cut pieces also do not fall off (Fig.~\ref{fig:sawyer-tasks}(b)). This is a task which requires complex maneuvers to successfully cut the fruit pieces. This is representative of complex manipulation tasks where the trajectory path and forces applied can matter for successfully achieving the goal.

\begin{table}[htb]
    \centering
    \caption{Ordered subtask categories
    of the box opening task.}
    \begin{tabular}{|c|c|}
    \hline
    Index & Subtask Category\\
    \hline\hline
    1 & Move arm towards the lid on the closed box\\
    \hline
    2 & Click button to open the lid of the box \\
    \hline
    3 & Grasp button on the lid of the box \\
    \hline
    4 & Transport the lid from the box towards table\\
    \hline
    5 & Release the button of the lid on the table from the gripper\\
    \hline
    6 & Move arm towards the green object that's inside the box\\
    \hline
    7 & Grasp the green object\\
    \hline
    8 & \specialcell{Transport the green object from\\ inside the box towards the table}\\
    \hline
    9 & Release the green object from gripper\\
    \hline
    10 & Move arm towards the lid on the table\\
    \hline
    11 & Grasp the button of the lid placed on the table\\
    \hline
    12 & Transport the lid from the table towards the box's body\\
    \hline
    13 & \specialcell{Release the button of the lid\\ on top of the box from the gripper}\\
    \hline
    14 & Push the button to lock lid\\
    \hline
    15 & Move arm towards green object\\
    \hline
    16 & Grasp green object on the table\\
    \hline
    17 & Transport the green object towards lid button \\
    \hline
    18 & Release the green object from gripper on top of the lid\\
    \hline
    \end{tabular}
    \label{tab:box_seg_labels}
    % \vspace{-2mm}
\end{table}

\subsection{Robot System}
\label{sec:system}

Demonstrations were provided to a 7 degree-of-freedom Sawyer manipulator with series elastic actuators and a parallel gripper. We used
a Movo MC1000 Conference USB microphone to record audio during demonstrations. All  participants were told that the robot can watch and listen to them. 
We used three static camera sensors (facing the human demonstrator and workspace) to collect high resolution video
data at $\sim\hspace{-1.5mm}10$ Hz for observing the demonstration. 
The recorded visual and audio data were synchronized and collected using ROS~\cite{quigley2009ros}. 


\begin{table}[htb]
    \centering
    \caption{Ordered subtask categories
    of the fruit cutting task.}
    \begin{tabular}{|c|c|}
    \hline
    Index & Subtask Category\\
    \hline\hline
    1 & Move arm towards the knife\\
    \hline
    2 & Grasp the knife while it's inside the knife holder\\
    \hline
    3 & Move the knife out from knife holder \\
    \hline
    4 & \specialcell{Transport knife from the \\knife holder towards the banana}\\
    \hline
    5 & Cut the first piece of the banana\\
    \hline
    6 & Cut the second piece of the banana\\
    \hline
    7 & \specialcell{Transport knife back from the\\ cutting board to the knife holder}\\
    \hline
    8 & Place the knife back in the knife holder\\
    \hline
    9 & Release the knife from the gripper\\
    \hline
    \end{tabular}
    \label{tab:cutting_seg_labels}
    % \vspace{-5mm}
\end{table}


\subsection{User Study}
\label{sec:user-study}
\subsubsection{Independent Variables (IVs)}
\label{sec:IVs}
We evaluated the effects of two independent variables (demonstration type and instruction type) on different acoustic features. For demonstration type (within-subjects), we focus on two modalities of LfD for robot manipulation \cite{kroemer2019review}: (1) learning via kinesthetic teaching (KT) in which the joints of a robot are moved along a trajectory in order to accomplish the task \cite{akgun2012trajectories}, and (2) learning from observation, specifically video demonstrations, in which a robot passively observes a human performing the task. For instruction type (between-subjects), we focused on the narration and natural conditions. Half of the participants were part of the narration condition, in which they were explicitly asked to use speech to communicate their intentions as they demonstrate. The remaining half of the participants were in the natural condition, in which they were only told that the robot can listen to them but not asked to use speech specifically. To analyze data for subtasks and errors during demonstrations, an IV indicating their presence or absence is used (example of presence/absence depicted in Fig.~\ref{fig:seg_errors}).


\subsubsection{Data Collection Procedure}
We collected demonstration data from 20 participants (8 males, 12 females) for each of the two tasks (Fig. \ref{fig:sawyer-tasks}). Participants were graduate or undergraduate students, recruited from a university campus. All participants used English speech and were %comfortable
proficient at speaking the language. Each participant was 
allowed one practice round for each demonstration type on the task they were assigned to do first. After one round of practicing, participants completed 2 demonstrations (1 KT, 1 video) for the box opening task and 2 demonstrations (1 KT, 1 video) for the fruit cutting task. The order of tasks and demonstration types were counterbalanced across all participants. 
We discarded data from two participants due to network issues during recording and perform our analysis on the remaining 18 participants. This amounted to a total of $\sim$24 minutes of video demonstration data and $\sim$119 minutes of KT demonstration data. 


\subsubsection{Dependent Measures (DMs)}
\label{sec:dv}
Our dependent measures are the (1) duration %speech 
of utterances during demonstrations (also measured as speech density, i.e. fraction of a demonstration accompanied by speech), (2) acoustic features capturing the prosody of speech, and (3) richness of the content conveyed by %audio 
utterances. Richness of the content refers to the diversity of the concepts conveyed via the spoken words. 

\subsubsection{Research Hypotheses}
Our research hypotheses are as follows:
\begin{itemize}
    \item \textbf{H1}: Prior work has shown that humans rely more on additional channels of communicating intent, such as audio, during challenging tasks \cite{oviatt2004we}. Based on this finding and given the complexity of our manipulation tasks, we hypothesize that teachers would rely on using  %speech
    similar amount (speech density) and kind of
    utterances (expressiveness or prosody) under both the natural and narration instruction conditions.
    \item \textbf{H2}: Following the previous motivation from \cite{oviatt2004we}---since kinesthetic demonstrations require more physical effort from the human teacher compared to video demonstrations \cite{fischer2016comparison}, %,sena2020quantifying},
    we hypothesize that more pronounced acoustic features and higher density of speech would be present during kinesthetic demonstrations.
    \item \textbf{H3}: 
    Prior work which studied unrestricted audio signals in human tutoring from parents to children %, such as Schillingmann et al. 
    \cite{schillingmann2009computational}, established that human speech from the demonstrator binds to action events, with structured pauses between events.
    Given these findings, we hypothesize that human teachers' speech 
    would be more pronounced in terms of density and prosodic features \textit{during} relevant subtask executions in a demonstration (presence), compared to periods of gaps between subtasks (absence). 
    \item \textbf{H4}: Human %audio 
    utterances have been shown to be beneficial for improving the error prediction of ASR systems \cite{hirschberg2004prosodic}, with more emphatic uses of speech when errors occur. Thus, we hypothesize that human teachers' speech would be more expressive and emphatic during presence of error segments versus in their absence.
\end{itemize}







\subsection{Data Annotation} 
\label{sec:annotation}

Automated speech detection and recognition is an active and challenging research area \cite{yu2016automatic, juang2005automatic, benzeghiba2007automatic}.
Average word error rates on our dataset (computed using the publicly available Google Speech to Text API~\cite{googlestt}) are 0.37 (video demos) and 0.59 (KT demos).
To accurately characterize human speech, subtasks, and errors during demonstrations, we collected detailed annotations from three different human annotators. 
All annotators were undergraduate students recruited at a university campus. The following annotations were collected for each utterance (separated by a significant pause, as judged by the annotators.): start time, stop time, and speech transcription. %A speech segment is classified as an `utterance' if it is well-separated from another speech segment by a significant pause, as judged by the annotators.
Each annotation was provided via a GUI interface %$^{1}$
with information available from the audio microphone and all three camera views to be played back at any time. 

\begin{table}[htb]
    \centering
    \caption{Unordered error categories
    of the box opening and fruit cutting tasks.}
    \begin{tabular}{|c|c|}
    \hline
    Index & Error Category\\
    \hline\hline
    1 & \specialcell{Teacher forgets to perform\\ a step of the task}\\
    \hline
    2 & \specialcell{Teacher struggles to move the\\ robot's arm in a certain way (KT only)}\\
    \hline
    3 & \specialcell{Teacher struggles to grasp an object} %using the robot's gripper 
    \\
    \hline
    4 & \specialcell{Robot/Human arm collides with, knocks off,\\ or moves items from their original position}\\
    \hline
    5 & \specialcell{Teacher performs a step of\\ the task in the wrong order}\\
    \hline
    6 & \specialcell{Teacher unintentionally uses two hands\\ instead of one to perform the task (video only)}\\
    \hline
    7 & \specialcell{Teacher uses their human hand during a kinesthetic\\demonstration to complete the task/help the robot (KT only)}\\
    \hline
    8 & \specialcell{Teacher accidentally drops an object\\ already grasped by the robot's gripper (KT only)}\\
    \hline
    9 & \specialcell{Teacher intentionally re-strategizes\\ or re-attempts a step of the task} \\
    \hline
    10 & \specialcell{Unsuccessful step execution e.g. not applying\\ enough force with the knife to completely cut the banana}
    \\
    \hline
    11 & Other\\
    \hline
    \end{tabular}
    \label{tab:err_labels}
    % \vspace{-3mm}
\end{table}



Annotators also separately marked the start and end times of predefined error and 
subtask categories for each demonstration (Fig. \ref{fig:seg_errors}), along with labels of predefined speech categories present with each identified subtask and error. 
The predefined subtask categories 
are listed in Table~\ref{tab:box_seg_labels} for the box opening task 
and in Table~\ref{tab:cutting_seg_labels} for the fruit cutting task. 
Each subtask category represents a primitive step that a robot can learn a policy for. 
% Prior works have shown that %it is important to segment a complex task into simpler subtasks, and then learn subsequent policies for each subtask. It has been shown that
% learning a separate policy for each step of a task can lead to improved generalization \cite{niekum2012learning,konidaris2012robot}.
The predefined error categories for both tasks are listed in Table~\ref{tab:err_labels}.  
The predefined speech categories that were labeled along with subtask and error instances were: (1) frustration, (2) encouragement, (3) speech pauses (explicit pause or filler words between two speech utterances), (4) laughter, (5) surprise, (6) no variation in manner of speech (normal). Annotators could also choose to label an utterance in a `none' category if it did fit well under any of the predefined categories. All predefined categories were determined following the methodology of grounded theory analysis \cite{charmaz2007grounded,charmaz2014constructing,morse2016developing}. 



\subsection{Acoustic Feature Computation}
\label{sec:features}

We compute several acoustic features over the annotated utterances to characterize prosody and content of human speech.  
We first processed raw audio signals of human demonstrators with a speech enhancement model~\cite{defossez2020real} to filter out the effect of environmental object-interaction sounds and robot motor noises. We then compute 10 %different
hand-crafted prosodic features (Audio II) %to study audio patterns --- 
to capture prosody and affect in terms of variation in the loudness or speed with which a speaker can alter their pronouncement of an utterance \cite{hirschberg2004prosodic,tran2017parsing,kim2007learning,short2018detecting,kim2018crepe} 
--- %speech duration; 
maximum pitch, energy, and loudness; mean pitch, energy, and loudness; 
total energy;
pause duration between speech acts; total word count and word rate. Pitch, loudness, and energy features represent measures of intonation and enunciation, whereas duration, pause, word count, word rate capture timing information. 
These hand-crafted acoustic features have been shown to enhance semantic parsing \cite{tran2017parsing}, understand speech recognition failures in dialogue systems \cite{hirschberg2004prosodic}, and widely used for applications in  human-robot interaction~\cite{kim2009people,short2018detecting} and speech recognition~\cite{yu2016automatic} communities. 

\begin{table}
    \centering
    \caption{Percentage of a demonstration duration accompanied by utterances (speech density), subtasks, and errors. Aggregate statistics (mean \& standard error) are reported for each of the four subsets resulting from two IVs. 
    }
    \begin{tabular}{|c|c|c|c|}
    \hline
    \begin{tabular}[c]{@{}c@{}}Demo Type/\\Instruction Type\end{tabular} & \%Utterances & \%Subtasks & \%Errors \\
    \hline\hline
    Video/Natural  & $57.97 \pm 14.12$ & $79.56 \pm 1.80$  & $9.09 \pm 3.27$  \\
    \hline
    Video/Narration & $89.89 \pm 3.26$  & $90.67 \pm 2.28$  & $4.84 \pm 1.87$   \\
    \hline
    KT/Natural & $27.90 \pm 11.86$ & $91.43 \pm 2.41$  & $20.01 \pm 3.87$  \\
    \hline
    KT/Narration & $71.60 \pm 6.09$  & $85.33 \pm 2.95$  & $24.57 \pm 2.74$ \\
    \hline
    \end{tabular}
    \label{tab:stats}
    % \vspace{-5mm}
\end{table}






\begin{comment}
It is important to note that such features computed within or around audio utterances %such as pause, duration %and other relevant features within active speech acts
are typically used when accurate annotations for audio utterances are available (as is often the case with large scale datasets used for automatic speech recognition and its applications). Hence, annotating our user study data was critical to perform detailed and accurate analysis. 
\end{comment}



We also analyze annotated prosodic features (Audio I) in the form of  emotion labels present in speech %during subtasks and errors 
(Sec.~\ref{sec:annotation}). In addition to the annotated (Audio I) and hand-crafted acoustic features (Audio II), we also compute 256-dimensional deep acoustic features (PASE~\cite{pascual2019learning}) for our learning experiments (Sec.~\ref{sec:learning-method}). PASE features are obtained from the last layer of a problem-agnostic speech encoder, trained in a self-supervised manner, and beneficial for downstream tasks which leverage speech features. %\as{More description about how PASE is trained and used}. 
To understand the richness of semantic content conveyed via audio utterances, we used variance of GloVe embeddings \cite{pennington2014glove} (first principal component from PCA analysis) for words in the annotated speech transcriptions.  
GloVe embeddings are word representations that capture fine-grained semantic and syntactic regularities of words using vector arithmetic.
The variance of such embeddings %vectors
can quantify the variety of concepts communicated.


\subsection{Learning Classifiers for Subtask and Error Detection}
\label{sec:learning-method}

To further understand if different acoustic features in human speech can identify subtasks and errors during demonstrations, we use random forest classifiers ~\cite{pedregosa2011scikit} for two binary classification tasks: (1) subtask detection and (2) error detection. 
The default implementation from the scikit-learn Python library~\cite{pedregosa2011scikit} is used for our experiments.
We use $100$ trees for each experiment. From the human facing camera, we also sample every $16^{th}$ frame
to compute video features (penultimate layer output of I3D~\cite{carreira2017quo} pretrained on the Kinetics activity recognition dataset~\cite{kay2017kinetics}) and corresponding audio features (Sec.~\ref{sec:features}) for a 1 second window around this frame. 
This provides about $2000$ (cutting) and
$2500$ (box) samples for kinesthetic demonstrations; and $370$ (cutting) and 
$510$ (box) samples for video demonstrations. Audio features consist of annotated speech labels encoded as one-hot vectors (Audio I) described in Sec.~\ref{sec:annotation}, hand-crafted prosodic features (Audio II) described in Sec.~\ref{sec:features}, as well as deep acoustic features (PASE~\cite{pascual2019learning}). 
